Plannable Approximations to MDP Homomorphisms: Equivariance under Actions

This work exploits action equivariance for representation learning in reinforcement learning. Equivariance under actions states that transitions in the input space are mirrored by equivalent transitions in latent space, while the map and transition functions should also commute. We introduce a contrastive loss function that enforces action equivariance on the learned representations. We prove that when our loss is zero, we have a homomorphism of a deterministic Markov Decision Process (MDP). Learning equivariant maps leads to structured latent spaces, allowing us to build a model on which we plan through value iteration. We show experimentally that for deterministic MDPs, the optimal policy in the abstract MDP can be successfully lifted to the original MDP. Moreover, the approach easily adapts to changes in the goal states. Empirically, we show that in such MDPs, we obtain better representations in fewer epochs compared to representation learning approaches using reconstructions, while generalizing better to new goals than model-free approaches.

==> discussion.tex <==
We have presented here a way of learning homomorphisms of MDPs. Our current approach relies on having some behavior policy sample a good spread of the true MDP's state and action space. This assumption may hold in certain cases, such as those where we can generalize from earlier instances of the problem (such as our amortized planning experiment) or when there is a lot of historical data available. However, our current approach side-steps the issue of scaling and exploration. For exploration, an approach may be based on one of the many model-based approaches there are, e.g. ensembles of models. However, for real scalability we should like to perform some clustering in the learned latent space. The issue is that end-to-end clustering in deep learning does not work reliably well (we have played around with this). For future work we would like to adapt our current approach to encourage latent states to cluster together based on bisimulation metrics~\cite{}. 
